Emergence of Nestedness in the Public Internet Peering Ecosystem

Nestedness is a property of bipartite complex networks that has been shown to characterize the peculiar structure of biological and economical networks. In a nested network, a node of low degree has its neighborhood included in the neighborhood of nodes of higher degree. Emergence of nestedness is commonly due to two different schemes: i) mutualistic behavior of nodes, where nodes of each class have an advantage in associating with each other, such as plant pollination or seed dispersal networks; ii) geographic distribution of species, captured in a so-called biogeographic network where species represent one class and geographical areas the other one. Nestedness has useful applications on real-world networks such as node ranking and link prediction. Motivated by analogies with biological networks, we study the nestedness property of the public Internet peering ecosystem, an important part of the Internet where autonomous systems (ASes) exchange traffic at Internet eXchange Points (IXPs). We propose two representations of this ecosystem using a bipartite graph derived from PeeringDB data. The first graph captures the AS [is member of] IXP relationship which is reminiscent of the mutualistic networks. The second graph groups IXPs into countries, and we define the AS [is present at] country relationship to mimic a biogeographic network. We statistically confirm the nestedness property of both graphs, which has never been observed before in Internet topology data. From this unique observation, we show that we can use node metrics to extract new key ASes and make efficient prediction of newly created links over a two-year period.

==> tabPeeringDima_ASesRanks.tex <==
\begin{table}[]
\centering
\resizebox{.98\textwidth}{!}{%
\begin{tabular}{@{}l|l|l|l@{}}
\toprule
 &
  Degree &
  Fitness &
  Binmatnest \\ \midrule
1 &
  Packet Clearing House &
  Packet Clearing House {[}0{]} &
  Packet Clearing House {[}0{]} \\
2 &
  Packet Clearing House AS42 &
  Packet Clearing House AS42 {[}0{]} &
  Packet Clearing House AS42 {[}0{]} \\
3 &
  Cloudflare &
  Cloudflare {[}0{]} &
  Facebook Inc AS63293 {[}14{]} \\
4 &
  Akamai Technologies &
  Facebook Inc AS63293 {[}13{]} &
  Cloudflare {[}-1{]} \\
5 &
  Hurricane Electric &
  Akamai Technologies {[}-1{]} &
  Akamai Technologies {[}-1{]} \\
6 &
  VeriSign Global Registry Services &
  Hurricane Electric {[}-1{]} &
  VeriSign Global Registry Services {[}0{]} \\
7 &
  Microsoft &
  VeriSign Global Registry Services {[}-1{]} &
  Hurricane Electric {[}-2{]} \\
8 &
  Facebook Inc &
  RIPE NCC K-Root Operations {[}5{]} &
  Google LLC {[}1{]} \\
9 &
  Google LLC &
  Netnod {[}2{]} &
  Netnod {[}2{]} \\
10 &
  Amazon.com &
  Facebook Inc {[}-2{]} &
  RIPE NCC K-Root Operations {[}3{]} \\
11 &
  Netnod &
  Google LLC {[}-2{]} &
  Facebook Inc {[}-3{]} \\
12 &
  Subspace &
  Microsoft {[}-5{]} &
  Microsoft {[}-5{]} \\
13 &
  RIPE NCC K-Root Operations &
  Amazon.com {[}-3{]} &
  Amazon.com {[}-3{]} \\
14 &
  Imperva &
  HUAWEI CLOUD {[}33{]} &
  Subspace {[}-2{]} \\
15 &
  Netflix &
  Netskope {[}12{]} &
  Netskope {[}12{]} \\
16 &
  Anexia &
  Subspace {[}-4{]} &
  Verizon Digital Media Services (EdgeCast Networks) {[}13{]} \\
17 &
  Facebook Inc AS63293 &
  Verizon Digital Media Services (EdgeCast Networks) {[}12{]} &
  Limelight Networks Global {[}7{]} \\
18 &
  Riot Games &
  Open Peering {[}87{]} &
  Netflix {[}-3{]} \\
19 & G-Core Labs & Global Cloud Xchange (f.k.a. FLAG Telecom) {[}55{]} & SoftLayer Technologies, Inc. (an IBM Company) {[}38{]} \\
20 &
  Yahoo! &
  Netflix {[}-5{]} &
  G-Core Labs {[}-1{]} \\
21 &
  Valve Corporation &
  Blizzard Entertainment {[}28{]} &
  HUAWEI CLOUD {[}26{]} \\
22 &
  SG.GS &
  Limelight Networks Global {[}2{]} &
  Anexia {[}-6{]} \\
23 &
  Zenlayer Inc &
  G-Core Labs {[}-4{]} &
  Wnet Telecom USA {[}42{]} \\
24 &
  Limelight Networks Global &
  Riot Games {[}-6{]} &
  SG.GS {[}-2{]} \\
25 &
  Swisscom &
  Vodafone Global Network {[}43{]} &
  Riot Games {[}-7{]} \\
26 &
  M247 &
  Anexia {[}-10{]} &
  Valve Corporation {[}-5{]} \\
27 &
  Netskope &
  SoftLayer Technologies, Inc. (an IBM Company) {[}30{]} &
  Quantil Networks {[}1{]} \\
28 &
  Quantil Networks &
  Imperva {[}-14{]} &
  Imperva {[}-14{]} \\
29 &
  Verizon Digital Media Services (EdgeCast Networks) &
  Valve Corporation {[}-8{]} &
  OVHcloud {[}9{]} \\
30 &
  Equinix Internet Exchange - MLPE &
  Quantil Networks {[}-2{]} &
  RETN {[}14{]} \\
31 &
  Telekomunikasi Indonesia Int (TELIN) &
  Wnet Telecom USA {[}34{]} &
  Global Cloud Xchange (f.k.a. FLAG Telecom) {[}43{]} \\
32 &
  Fastly, Inc. &
  SG.GS {[}-10{]} &
  Dropbox {[}32{]} \\
33 &
  i3D.net &
  Twitch {[}1{]} &
  M247 {[}-7{]} \\
34 &
  Twitch &
  OVHcloud {[}4{]} &
  Yahoo! {[}-14{]} \\
35 &
  StackPath (Highwinds) &
  i3D.net {[}-2{]} &
  Equinix Internet Exchange - MLPE {[}-5{]} \\
36 &
  Colt &
  Equinix Internet Exchange - MLPE {[}-6{]} &
  Telekomunikasi Indonesia Int (TELIN) {[}-5{]} \\
37 &
  IPTP Networks &
  M247 {[}-11{]} &
  IX Reach {[}18{]} \\
38 &
  OVHcloud &
  Dropbox {[}26{]} &
  NetIX Communications Ltd. {[}8{]} \\
39 &
  Forcepoint Cloud &
  Saudi Telecom Company (STC IGW) {[}31{]} &
  i3D.net {[}-6{]} \\
40 &
  Cisco Umbrella &
  Yahoo! {[}-20{]} &
  Swisscom {[}-15{]} \\
41 &
  NetActuate &
  Fastly, Inc. {[}-9{]} &
  Zenlayer Inc {[}-18{]} \\
42 &
  BT &
  RETN {[}2{]} &
  Twitch {[}-8{]} \\
43 &
  Alibaba Cloud CDN &
  Zenlayer Inc {[}-20{]} &
  Fastly, Inc. {[}-11{]} \\
44 &
  RETN &
  Swisscom {[}-19{]} &
  EdgeUno {[}59{]} \\
45 &
  DNS-OARC-112 &
  Telekomunikasi Indonesia Int (TELIN) {[}-14{]} &
  Saudi Telecom Company (STC IGW) {[}25{]} \\
46 &
  NetIX Communications Ltd. &
  EdgeUno {[}57{]} &
  RouteIX Networks {[}26{]} \\
47 &
  HUAWEI CLOUD &
  IX Reach {[}8{]} &
  Open Peering {[}58{]} \\
48 &
  Apple Inc. &
  RouteIX Networks {[}24{]} &
  Alibaba Cloud CDN {[}-5{]} \\
49 &
  Blizzard Entertainment &
  NetIX Communications Ltd. {[}-3{]} &
  Colt {[}-13{]} \\
50 &
  CacheFly &
  Colt {[}-14{]} &
  Unitas Global {[}13{]} \\ \bottomrule
\end{tabular}}
\caption{\autoref{fig:peeringDima_packing} row nodes rankings. Difference in rankings w.r.t. to DegreeRank is given in brackets.}
\label{tab:peeringDima_ASesRanks}
\end{table}

==> tabPeeringDima_ASesRanks1000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lllll@{}}
\toprule
   & Degree\_country & Complexity  & Degree\_AS                           & Fitness                                       \\ \midrule
1  & DE              & DE {[}0{]}  & Packet Clearing House                & Packet Clearing House {[}0{]}                 \\
2  & US              & US {[}0{]}  & Packet Clearing House AS42           & Packet Clearing House AS42 {[}0{]}            \\
3  & NL              & NL {[}0{]}  & Cloudflare                           & Facebook Inc AS63293 {[}14{]}                 \\
4  & GB              & GB {[}0{]}  & Akamai Technologies                  & Akamai Technologies {[}0{]}                   \\
5  & BR              & BR {[}0{]}  & Hurricane Electric                   & Cloudflare {[}-2{]}                           \\
6  & FR              & FR {[}0{]}  & VeriSign Global Registry Services    & Nexusguard Limited {[}232{]}                  \\
7  & SG              & SG {[}0{]}  & Microsoft                            & VeriSign Global Registry Services {[}-1{]}    \\
8  & HK              & HK {[}0{]}  & Facebook Inc                         & Hurricane Electric {[}-3{]}                   \\
9  & RU              & RU {[}0{]}  & Google LLC                           & RIPE NCC K-Root Operations {[}4{]}            \\
10 & JP              & JP {[}0{]}  & Amazon.com                           & Core-Backbone {[}66{]}                        \\
11 & AU              & AU {[}0{]}  & Netnod                               & Facebook Inc {[}-3{]}                         \\
12 & CH              & CH {[}0{]}  & Subspace                             & Netnod {[}-1{]}                               \\
13 & SE              & SE {[}0{]}  & RIPE NCC K-Root Operations           & Sprint {[}132{]}                              \\
14 & CA              & CA {[}0{]}  & Imperva                              & Google LLC {[}-5{]}                           \\
15 & ZA              & ZA {[}0{]}  & Anexia                               & Microsoft {[}-8{]}                            \\
16 & IT              & IT {[}0{]}  & Netflix                              & Equinix Internet Exchange - MLPE {[}14{]}     \\
17 & ES              & ES {[}0{]}  & Facebook Inc AS63293                 & MBIX Route Servers {[}1268{]}                 \\
18 & PL              & PL {[}0{]}  & Yahoo!                               & Univision Mongolia {[}1275{]}                 \\
19 & CZ & CZ {[}0{]}  & Valve Corporation                                  & S-IT Informationstechnologie Betreiber GmbH \& Co. KG {[}1300{]} \\
20 & ID              & ID {[}0{]}  & Riot Games                           & Netskope {[}8{]}                              \\
21 & IN              & IN {[}0{]}  & G-Core Labs                          & Amazon.com {[}-11{]}                          \\
22 & UA              & UA {[}0{]}  & SG.GS                                & Vodacom {[}362{]}                             \\
23 & RO              & RO {[}0{]}  & Zenlayer Inc                         & ELETRONET {[}362{]}                           \\
24 & AT              & AT {[}0{]}  & Swisscom                             & Dropbox {[}42{]}                              \\
25 & BG & BG {[}0{]}  & Limelight Networks Global                          & Capital Online Data Service Ltd {[}77{]}                         \\
26 & IE              & IE {[}0{]}  & M247                                 & Fiber Telecom Italia {[}157{]}                \\
27 & DK              & DK {[}0{]}  & Quantil Networks                     & Subspace {[}-15{]}                            \\
28 & AE              & KR {[}1{]}  & Netskope                             & Zayo France {[}94{]}                          \\
29 & KR & AE {[}-1{]} & Verizon Digital Media Services (EdgeCast Networks) & VOXILITY {[}129{]}                                               \\
30 & TH              & TH {[}0{]}  & Equinix Internet Exchange - MLPE     & Olivenet Network {[}201{]}                    \\
31 & NZ              & NZ {[}0{]}  & Fastly, Inc.                         & Acquire Asia Pacific {[}331{]}                \\
32 & TW              & PT {[}1{]}  & Telekomunikasi Indonesia Int (TELIN) & Norlys Tele {[}452{]}                         \\
33 & PT              & TW {[}-1{]} & i3D.net                              & Hivane {[}254{]}                              \\
34 & MY              & MY {[}0{]}  & Twitch                               & VNIX-HCM Route Servers {[}1202{]}             \\
35 & NO              & NO {[}0{]}  & StackPath (Highwinds)                & Teknologi Bumi Nusantara {[}1202{]}           \\
36 & AR              & AR {[}0{]}  & IPTP Networks                        & ACORUS NETWORKS {[}60{]}                      \\
37 & LU              & LU {[}0{]}  & Colt                                 & Alanyhq Networks Limited {[}49{]}             \\
38 & FI              & FI {[}0{]}  & BT                                   & Liquid Telecommunications Ltd {[}57{]}        \\
39 & SK              & SK {[}0{]}  & Forcepoint Cloud                     & Sunrise Communications AG {[}189{]}           \\
40 & CL              & CL {[}0{]}  & NetActuate                           & UpCloud {[}293{]}                             \\
41 & CN              & CN {[}0{]}  & Cisco Umbrella                       & Riot Games {[}-21{]}                          \\
42 & TR              & TR {[}0{]}  & OVHcloud                             & Kevin Buehl AS35619 {[}195{]}                 \\
43 & BE              & BE {[}0{]}  & Alibaba Cloud CDN                    & SEACOM {[}109{]}                              \\
44 & GR              & GR {[}0{]}  & RETN                                 & SG.GS {[}-22{]}                               \\
45 & HU              & HU {[}0{]}  & DNS-OARC-112                         & Cool Ideas Service Provider Pty Ltd {[}603{]} \\
46 & NG              & LV {[}2{]}  & NetIX Communications Ltd.            & China Mobile International {[}60{]}           \\
47 & KE              & NG {[}-1{]} & Apple Inc.                           & Defense.Net {[}520{]}                         \\
48 & LV              & KE {[}-1{]} & Alibaba                              & Anexia {[}-33{]}                              \\
49 & EE              & EE {[}0{]}  & HUAWEI CLOUD                         & Fibrenoire {[}773{]}                          \\
50 & RS              & RS {[}0{]}  & Blizzard Entertainment               & G-Core Labs {[}-29{]}                         \\ \bottomrule
\end{tabular}
\end{table}

==> tabPeeringDima_ASesRanks10000Comp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\resizebox{.98\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
 &
  Degree &
  Fitness &
  Binmatnest \\ \midrule
1 &
  Packet Clearing House &
  Packet Clearing House {[}0{]} &
  Packet Clearing House {[}0{]} \\
2 &
  Packet Clearing House AS42 &
  Packet Clearing House AS42 {[}0{]} &
  Packet Clearing House AS42 {[}0{]} \\
3 &
  Cloudflare &
  Facebook Inc AS63293 {[}14{]} &
  Cloudflare {[}0{]} \\
4 &
  Akamai Technologies &
  Cloudflare {[}-1{]} &
  Akamai Technologies {[}0{]} \\
5 &
  Hurricane Electric &
  Akamai Technologies {[}-1{]} &
  Facebook Inc AS63293 {[}12{]} \\
6 &
  VeriSign Global Registry Services &
  3P System Srl {[}1291{]} &
  VeriSign Global Registry Services {[}0{]} \\
7 &
  Microsoft &
  HKBN Enterprise Solutions HK Limited {[}239{]} &
  Hurricane Electric {[}-2{]} \\
8 &
  Facebook Inc &
  BHTelecom {[}1109{]} &
  Netnod {[}3{]} \\
9 &
  Google LLC &
  Facebook Inc {[}-1{]} &
  Facebook Inc {[}-1{]} \\
10 &
  Amazon.com &
  VeriSign Global Registry Services {[}-4{]} &
  RIPE NCC K-Root Operations {[}3{]} \\
11 &
  Netnod &
  RIPE NCC K-Root Operations {[}2{]} &
  Google LLC {[}-2{]} \\
12 &
  Subspace &
  iNET Communications {[}1257{]} &
  Zayo France {[}124{]} \\
13 &
  RIPE NCC K-Root Operations &
  Netnod {[}-2{]} &
  Microsoft {[}-6{]} \\
14 &
  Imperva &
  Hurricane Electric {[}-9{]} &
  GTT (former KPN International / KPN Eurornigs) {[}411{]} \\
15 &
  Netflix &
  Continent 8 Technologies plc {[}65{]} &
  Orange Romania S.A. {[}432{]} \\
16 &
  Anexia &
  Netskope {[}10{]} &
  HKBN Enterprise Solutions HK Limited {[}230{]} \\
17 &
  Facebook Inc AS63293 &
  Zayo France {[}119{]} &
  Amazon.com {[}-7{]} \\
18 & G-Core Labs & GTT (former KPN International / KPN Eurornigs) {[}407{]} & Continent 8 Technologies plc {[}62{]} \\
19 &
  Valve Corporation &
  Orange Romania S.A. {[}428{]} &
  Subspace {[}-7{]} \\
20 &
  Riot Games &
  Google LLC {[}-11{]} &
  Netskope {[}6{]} \\
21 &
  Yahoo! &
  Cybersmart Ltd {[}1090{]} &
  Angola Cables {[}74{]} \\
22 &
  Limelight Networks Global &
  PP "New information systems" {[}1446{]} &
  iNET Communications {[}1247{]} \\
23 &
  Swisscom &
  Gilat Satcom {[}1447{]} &
  Equinix Internet Exchange - MLPE {[}6{]} \\
24 &
  SG.GS &
  PARABOLE REUNION {[}1569{]} &
  SkyCable Corporation {[}154{]} \\
25 &
  Zenlayer Inc &
  Fastic {[}4415{]} &
  Zoom Video Communications, Inc. {[}209{]} \\
26 &
  Netskope &
  LP PROVEDORA DE INTERNET E INSTALAÇÕES DE REDES TE {[}5304{]} &
  Quickline AG {[}934{]} \\
27 &
  Verizon Digital Media Services (EdgeCast Networks) &
  XCONNECT Chile {[}4824{]} &
  Wnet Telecom USA {[}39{]} \\
28 &
  M247 &
  Microsoft {[}-21{]} &
  10VPN Research Network {[}83{]} \\
29 &
  Equinix Internet Exchange - MLPE &
  SkyCable Corporation {[}149{]} &
  Filtiwan Network {[}1105{]} \\
30 &
  Quantil Networks &
  Quickline AG {[}930{]} &
  RIPE NCC RIS Project {[}24{]} \\
31 &
  Fastly, Inc. &
  Wnet Telecom USA {[}35{]} &
  Youssef Hamed {[}67{]} \\
32 &
  Telekomunikasi Indonesia Int (TELIN) &
  Zain Group - Wholesale {[}129{]} &
  LinzNet ISP GmbH {[}883{]} \\
33 &
  Twitch &
  10VPN Research Network {[}78{]} &
  Limelight Networks Global {[}-11{]} \\
34 &
  StackPath (Highwinds) &
  Amazon.com {[}-24{]} &
  Saudi Telecom Company (STC IGW) {[}48{]} \\
35 &
  i3D.net &
  HERE Global B.V. {[}305{]} &
  Valve Corporation {[}-16{]} \\
36 &
  Colt &
  Telikom PNG {[}1495{]} &
  3P System Srl {[}1261{]} \\
37 &
  IPTP Networks &
  Singapore Telecommunications Limited {[}217{]} &
  Bali Towerindo Sentra AS136119 {[}1207{]} \\
38 &
  OVHcloud &
  Zoom Video Communications, Inc. {[}196{]} &
  IXP Route Servers {[}112{]} \\
39 &
  Cisco Umbrella &
  DDoS-Guard.net main network {[}642{]} &
  AT\&T EMEA - AS2686 {[}54{]} \\
40 &
  BT &
  MARCHNET {[}4857{]} &
  HERE Global B.V. {[}300{]} \\
41 &
  NetActuate &
  iBloo {[}4408{]} &
  Elkdata {[}864{]} \\
42 &
  Forcepoint Cloud &
  ElecTower {[}4408{]} &
  TurkNet Iletisim Hizmetleri A.S {[}916{]} \\
43 &
  RETN &
  Polymer Network {[}4994{]} &
  netplus.ch {[}362{]} \\
44 &
  DNS-OARC-112 &
  TI SYSTEMS {[}4994{]} &
  Netflix {[}-29{]} \\
45 &
  Alibaba Cloud CDN &
  Subspace {[}-33{]} &
  PCCW Global {[}95{]} \\
46 &
  Alibaba &
  Equinix Internet Exchange - MLPE {[}-17{]} &
  Unitas Global {[}21{]} \\
47 &
  HUAWEI CLOUD &
  Filtiwan Network {[}1087{]} &
  LeaseWeb Network {[}63{]} \\
48 &
  Apple Inc. &
  LinzNet ISP GmbH {[}867{]} &
  Zain Group - Wholesale {[}113{]} \\
49 &
  Blizzard Entertainment &
  Angola Cables {[}46{]} &
  BHTelecom {[}1068{]} \\
50 &
  NetIX Communications Ltd. &
  igloo22225 - AS203729 {[}610{]} &
  Swisscom {[}-27{]} \\ \bottomrule
\end{tabular}}
\caption{Fitness-Complexity and Binmatnest rankings for the largest connected component in peeringDima. Here $\topN=10000$.}
\label{tab:PeeringDima_ASesRanks10000Comp}
\end{table}

==> tabPeeringDima_ASesRanks10000NoComp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table}[]
\resizebox{.98\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
   & Degree\_country & Complexity inv  & Degree\_AS                           & Fitness                                          \\ \midrule
1  & US              & US {[}0{]}  & Packet Clearing House                & Packet Clearing House {[}0{]}                    \\
2  & BR & BR {[}0{]} & Packet Clearing House AS42                         & Packet Clearing House AS42 {[}0{]}  \\
3  & DE              & DE {[}0{]}  & Cloudflare                           & Facebook Inc AS63293 {[}14{]}                    \\
4  & NL              & NL {[}0{]}  & Akamai Technologies                  & Cloudflare {[}-1{]}                              \\
5  & GB              & GB {[}0{]}  & Hurricane Electric                   & Akamai Technologies {[}-1{]}                     \\
6  & IN              & IN {[}0{]}  & VeriSign Global Registry Services    & IProute {[}1518{]}                               \\
7  & FR              & FR {[}0{]}  & Microsoft                            & Cisco Systems, Inc. {[}229{]}                    \\
8  & PL              & PL {[}0{]}  & Facebook Inc                         & Mass Response / spusu {[}1495{]}                 \\
9  & RU              & RU {[}0{]}  & Google LLC                           & Facebook Inc {[}-1{]}                            \\
10 & AU              & AU {[}0{]}  & Amazon.com                           & VeriSign Global Registry Services {[}-4{]}       \\
11 & ZA              & ZA {[}0{]}  & Netnod                               & Cloudata {[}1279{]}                              \\
12 & CA              & CA {[}0{]}  & Subspace                             & Netnod {[}-1{]}                                  \\
13 & SG              & SG {[}0{]}  & RIPE NCC K-Root Operations           & Hurricane Electric {[}-8{]}                      \\
14 & JP              & JP {[}0{]}  & Imperva                              & Tiggee {[}59{]}                                  \\
15 & IT              & IT {[}0{]}  & Netflix                              & Quantil Networks {[}15{]}                        \\
16 & ID              & ID {[}0{]}  & Anexia                               & RIPE NCC K-Root Operations {[}-3{]}              \\
17 & CH              & CH {[}0{]}  & Facebook Inc AS63293                 & RASCOM {[}98{]}                                  \\
18 & HK              & HK {[}0{]}  & Valve Corporation                    & Dolphin Telecom {[}402{]}                        \\
19 & AR              & AR {[}0{]}  & G-Core Labs                          & Acquire Asia Pacific {[}416{]}                   \\
20 & SE              & SE {[}0{]}  & Yahoo!                               & Google LLC {[}-11{]}                             \\
21 & ES              & ES {[}0{]}  & Riot Games                           & Bangladesh Telecommunications {[}1454{]}         \\
22 & UA              & UA {[}0{]}  & Limelight Networks Global            & iNET Communications {[}1662{]}                   \\
23 & CZ              & CZ {[}0{]}  & Zenlayer Inc                         & OtradnoeNet {[}1665{]}                           \\
24 & RO              & RO {[}0{]}  & Swisscom                             & Radiokomunikace {[}1626{]}                       \\
25 & AT              & AT {[}0{]}  & SG.GS                                & Nasional Online {[}4259{]}                       \\
26 & BG              & BG {[}0{]}  & Netskope                             & Andalas Media Informatika {[}5081{]}             \\
27 & CL & CL {[}0{]} & Verizon Digital Media Services (EdgeCast Networks) & Modern Networks Services {[}4894{]} \\
28 & NZ              & NZ {[}0{]}  & M247                                 & GILEADE TELECOMUNICACOES E MULTIMIDIA {[}4799{]} \\
29 & MY              & MY {[}0{]}  & Equinix Internet Exchange - MLPE     & MARTON {[}4833{]}                                \\
30 & IE              & TW {[}1{]}  & Quantil Networks                     & cloudinfrastack {[}4841{]}                       \\
31 & TW              & IE {[}-1{]} & Fastly, Inc.                         & Ehiweb {[}4847{]}                                \\
32 & NO              & NO {[}0{]}  & Telekomunikasi Indonesia Int (TELIN) & Microsoft {[}-25{]}                              \\
33 & DK              & DK {[}0{]}  & Twitch                               & Ooredoo Qatar formerly Qatar Telecom {[}124{]}   \\
34 & TH              & TH {[}0{]}  & StackPath (Highwinds)                & Seeweb {[}928{]}                                 \\
35 & AE              & CN {[}1{]}  & i3D.net                              & Verizon Business - EMEA {[}27{]}                 \\
36 & CN              & AE {[}-1{]} & IPTP Networks                        & TELE2 {[}142{]}                                  \\
37 & KR              & KR {[}0{]}  & Colt                                 & Choopa, LLC {[}75{]}                             \\
38 & BE              & BE {[}0{]}  & NetActuate                           & Amazon.com {[}-28{]}                             \\
39 & LU              & LU {[}0{]}  & BT                                   & FPT Telecom {[}379{]}                            \\
40 & PT              & PT {[}0{]}  & OVHcloud                             & Cloudbase {[}1640{]}                             \\
41 & SK              & SK {[}0{]}  & Cisco Umbrella                       & Telehouse {[}248{]}                              \\
42 & GR              & GR {[}0{]}  & Forcepoint Cloud                     & Foton Telecom CJSC {[}180{]}                     \\
43 & FI              & FI {[}0{]}  & Alibaba Cloud CDN                    & atom86 {[}675{]}                                 \\
44 & NG              & NG {[}0{]}  & RETN                                 & Superimagem Tecnologia em Eletrônica {[}5211{]}  \\
45 & HU              & HU {[}0{]}  & DNS-OARC-112                         & AIRNET Italy {[}4803{]}                          \\
46 & KE              & KE {[}0{]}  & Blizzard Entertainment               & Simm IT Services {[}4803{]}                      \\
47 & TR              & LV {[}1{]}  & NetIX Communications Ltd.            & Gelexiy Cab Net {[}4788{]}                       \\
48 & LV              & LT {[}1{]}  & Alibaba                              & Sri Ram Broadband Services {[}4788{]}            \\
49 & LT              & PH {[}1{]}  & Apple Inc.                           & Viriya Surya Abadi {[}4788{]}                    \\
50 & PH              & TR {[}-3{]} & CacheFly                             & Subspace {[}-38{]}                               \\ \bottomrule
\end{tabular}}
\caption{Fitness-Complexity rankings for $\topN=10000$ peeringDima network. Difference wrt Degree ranking is given in brackets.}
\label{tab:PeeringDima_ASesRanks10000NoComp}
\end{table}

==> tabPeeringDima_ASesRanks500.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lllll@{}}
\toprule
   & Degree\_country & Complexity  & Degree\_AS                           & Fitness                                                    \\ \midrule
1  & DE              & DE {[}0{]}  & Packet Clearing House                & Packet Clearing House {[}0{]}                              \\
2  & NL              & NL {[}0{]}  & Packet Clearing House AS42           & Packet Clearing House AS42 {[}0{]}                         \\
3  & US              & US {[}0{]}  & Cloudflare                           & Facebook Inc AS63293 {[}14{]}                              \\
4  & GB              & GB {[}0{]}  & Akamai Technologies                  & Akamai Technologies {[}0{]}                                \\
5  & FR              & FR {[}0{]}  & Hurricane Electric                   & Cloudflare {[}-2{]}                                        \\
6  & SG              & SG {[}0{]}  & VeriSign Global Registry Services    & RIPE NCC K-Root Operations {[}7{]}                         \\
7  & BR              & BR {[}0{]}  & Microsoft                            & Hurricane Electric {[}-2{]}                                \\
8  & JP              & JP {[}0{]}  & Facebook Inc                         & VeriSign Global Registry Services {[}-2{]}                 \\
9  & HK              & HK {[}0{]}  & Google LLC                           & FusedIT Trust {[}107{]}                                    \\
10 & RU              & RU {[}0{]}  & Amazon.com                           & Facebook Inc {[}-2{]}                                      \\
11 & AU              & AU {[}0{]}  & Netnod                               & Netnod {[}0{]}                                             \\
12 & SE              & SE {[}0{]}  & Subspace                             & NORDUnet {[}72{]}                                          \\
13 & CA              & CA {[}0{]}  & RIPE NCC K-Root Operations           & Google LLC {[}-4{]}                                        \\
14 & ES              & CH {[}1{]}  & Imperva                              & Microsoft {[}-7{]}                                         \\
15 & CH              & ES {[}-1{]} & Anexia                               & Psychz Networks {[}146{]}                                  \\
16 & IT              & IT {[}0{]}  & Netflix                              & Zayo France {[}98{]}                                       \\
17 & ZA              & ZA {[}0{]}  & Facebook Inc AS63293                 & Netskope {[}9{]}                                           \\
18 & CZ              & CZ {[}0{]}  & Valve Corporation                    & EPIX.Katowice-LOCAL {[}605{]}                              \\
19 & PL              & PL {[}0{]}  & Yahoo!                               & IPTP NETWORKS S.A.C. {[}608{]}                             \\
20 & IN              & IN {[}0{]}  & Riot Games                           & Amazon.com {[}-10{]}                                       \\
21 & RO              & RO {[}0{]}  & G-Core Labs                          & Verizon Digital Media Services (EdgeCast Networks) {[}8{]} \\
22 & AT              & UA {[}1{]}  & Limelight Networks Global            & Subspace {[}-10{]}                                         \\
23 & UA              & AT {[}-1{]} & Zenlayer Inc                         & CentralNic Anycast A {[}43{]}                              \\
24 & BG              & BG {[}0{]}  & Swisscom                             & KT Corporation (Korea Telecom) {[}214{]}                   \\
25 & IE              & IE {[}0{]}  & SG.GS                                & China Mobile International {[}74{]}                        \\
26 & ID              & ID {[}0{]}  & Netskope                             & GEANT IAS {[}69{]}                                         \\
27 & DK & DK {[}0{]} & Equinix Internet Exchange - MLPE                   & Virtual Technologies \& Solutions {[}71{]} \\
28 & KR              & KR {[}0{]}  & Quantil Networks                     & euNetworks Group {[}195{]}                                 \\
29 & AE & AE {[}0{]} & Verizon Digital Media Services (EdgeCast Networks) & Türk Telekom International {[}79{]}        \\
30 & MY              & MY {[}0{]}  & M247                                 & IELO {[}324{]}                                             \\
31 & TH              & TH {[}0{]}  & Fastly, Inc.                         & Equinix Metal {[}169{]}                                    \\
32 & NZ              & NZ {[}0{]}  & Telekomunikasi Indonesia Int (TELIN) & Alanyhq Networks Limited {[}62{]}                          \\
33 & PT              & PT {[}0{]}  & StackPath (Highwinds)                & Flys Interativa AS28663 {[}412{]}                          \\
34 & FI              & TW {[}1{]}  & i3D.net                              & Telekenex Inc {[}492{]}                                    \\
35 & TW              & FI {[}-1{]} & Twitch                               & Allegro.pl Poland {[}587{]}                                \\
36 & NO              & NO {[}0{]}  & IPTP Networks                        & Yandex {[}578{]}                                           \\
37 & LU              & LU {[}0{]}  & Colt                                 & G-Core Labs {[}-16{]}                                      \\
38 & SK              & SK {[}0{]}  & Forcepoint Cloud                     & Valve Corporation {[}-20{]}                                \\
39 & CL              & CL {[}0{]}  & OVHcloud                             & HUAWEI CLOUD {[}11{]}                                      \\
40 & BE              & BE {[}0{]}  & Cisco Umbrella                       & SG.GS {[}-15{]}                                            \\
41 & TR              & TR {[}0{]}  & NetActuate                           & Netflix {[}-25{]}                                          \\
42 & KE              & KE {[}0{]}  & BT                                   & SoftLayer Technologies, Inc. (an IBM Company) {[}16{]}     \\
43 & HU              & HU {[}0{]}  & RETN                                 & Anexia {[}-28{]}                                           \\
44 & GR              & CN {[}1{]}  & Alibaba Cloud CDN                    & Internap {[}236{]}                                         \\
45 & CN              & GR {[}-1{]} & DNS-OARC-112                         & Wnet Telecom USA {[}22{]}                                  \\
46 & RS              & RS {[}0{]}  & Blizzard Entertainment               & i3D.net {[}-12{]}                                          \\
47 & AR              & AR {[}0{]}  & Apple Inc.                           & WebEx Communications {[}138{]}                             \\
48 & EE              & EE {[}0{]}  & NetIX Communications Ltd.            & Imperva {[}-34{]}                                          \\
49 & NG              & LV {[}1{]}  & Alibaba                              & Convergenze S.p.A. {[}115{]}                               \\
50 & LV              & NG {[}-1{]} & HUAWEI CLOUD                         & Linkedin {[}117{]}                                         \\ \bottomrule
\end{tabular}
\end{table}

==> tabPeeringDima_ASesRanks5000.tex <==
\begin{table}[]
\begin{tabular}{lllll}
   & Degree\_country & Complexity  & Degree\_AS                           & Fitness                                          \\
1  & US              & US {[}0{]}  & Packet Clearing House                & Packet Clearing House {[}0{]}                    \\
2  & DE              & DE {[}0{]}  & Packet Clearing House AS42           & Packet Clearing House AS42 {[}0{]}               \\
3  & BR              & BR {[}0{]}  & Cloudflare                           & Facebook Inc AS63293 {[}14{]}                    \\
4  & NL              & NL {[}0{]}  & Akamai Technologies                  & Cloudflare {[}-1{]}                              \\
5  & GB              & GB {[}0{]}  & Hurricane Electric                   & Akamai Technologies {[}-1{]}                     \\
6  & PL & PL {[}0{]} & VeriSign Global Registry Services                  & VeriSign Global Registry Services {[}0{]}                                   \\
7  & FR              & FR {[}0{]}  & Microsoft                            & Robert Finze {[}1536{]}                          \\
8  & RU              & RU {[}0{]}  & Facebook Inc                         & Symphony IP Transit {[}218{]}                    \\
9  & AU              & AU {[}0{]}  & Google LLC                           & FSF Tecnologia {[}1207{]}                        \\
10 & SG              & SG {[}0{]}  & Amazon.com                           & Facebook Inc {[}-2{]}                            \\
11 & ZA              & ZA {[}0{]}  & Netnod                               & Hurricane Electric {[}-6{]}                      \\
12 & JP              & IN {[}1{]}  & Subspace                             & Netnod {[}-1{]}                                  \\
13 & IN              & JP {[}-1{]} & RIPE NCC K-Root Operations           & RIPE NCC K-Root Operations {[}0{]}               \\
14 & HK              & HK {[}0{]}  & Imperva                              & OceanIX Route Servers {[}1237{]}                 \\
15 & ID              & ID {[}0{]}  & Anexia                               & Equinix Connect - EMEA {[}62{]}                  \\
16 & CA              & CA {[}0{]}  & Netflix                              & CDN77 {[}105{]}                                  \\
17 & CH              & CH {[}0{]}  & Facebook Inc AS63293                 & M247 {[}9{]}                                     \\
18 & IT              & IT {[}0{]}  & Riot Games                           & Google LLC {[}-9{]}                              \\
19 & SE              & SE {[}0{]}  & Valve Corporation                    & Global Network Managment {[}321{]}               \\
20 & ES              & ES {[}0{]}  & Yahoo!                               & Free SAS {[}324{]}                               \\
21 & UA              & UA {[}0{]}  & G-Core Labs                          & Microsoft {[}-14{]}                              \\
22 & CZ              & CZ {[}0{]}  & Swisscom                             & ISKON INTERNET {[}1240{]}                        \\
23 & AR              & AR {[}0{]}  & SG.GS                                & Verizon Communications Inc. LATAM {[}1326{]}     \\
24 & RO & RO {[}0{]} & Zenlayer Inc                                       & Stichting Nationale Beheersorganisatie Internet Providers (NBIP) {[}1382{]} \\
25 & AT              & AT {[}0{]}  & Limelight Networks Global            & Tiernan OToole {[}1166{]}                        \\
26 & BG              & BG {[}0{]}  & M247                                 & Altercom-21 {[}3254{]}                           \\
27 & NZ              & NZ {[}0{]}  & Netskope                             & Avaya {[}3318{]}                                 \\
28 & CL              & CL {[}0{]}  & Equinix Internet Exchange - MLPE     & Deep Media {[}3819{]}                            \\
29 & IE & IE {[}0{]} & Verizon Digital Media Services (EdgeCast Networks) & Openfactory Services {[}3594{]}                                             \\
30 & TW              & TW {[}0{]}  & Quantil Networks                     & TELCOCOM {[}3594{]}                              \\
31 & DK              & DK {[}0{]}  & Fastly, Inc.                         & Rocking Connect {[}3814{]}                       \\
32 & TH              & TH {[}0{]}  & Telekomunikasi Indonesia Int (TELIN) & Keepit UK-LD {[}3823{]}                          \\
33 & NO              & NO {[}0{]}  & i3D.net                              & Netskope {[}-6{]}                                \\
34 & AE              & AE {[}0{]}  & Twitch                               & Amazon.com {[}-24{]}                             \\
35 & KR              & KR {[}0{]}  & StackPath (Highwinds)                & BIGO {[}149{]}                                   \\
36 & MY              & MY {[}0{]}  & IPTP Networks                        & Orange Business Services Latin America {[}919{]} \\
37 & CN              & CN {[}0{]}  & Colt                                 & HKBN Enterprise Solutions HK Limited {[}207{]}   \\
38 & PT              & PT {[}0{]}  & OVHcloud                             & Subspace {[}-26{]}                               \\
39 & LU              & LU {[}0{]}  & NetActuate                           & Verizon Business - EMEA {[}26{]}                 \\
40 & SK              & SK {[}0{]}  & Cisco Umbrella                       & ip-it consult GmbH {[}66{]}                      \\
41 & FI              & FI {[}0{]}  & Forcepoint Cloud                     & Alex Delporte {[}132{]}                          \\
42 & GR              & GR {[}0{]}  & BT                                   & Asia Pacific Telecom {[}893{]}                   \\
43 & BE              & BE {[}0{]}  & DNS-OARC-112                         & Dolphin Telecom {[}308{]}                        \\
44 & NG              & NG {[}0{]}  & RETN                                 & RBMNET {[}1513{]}                                \\
45 & KE              & HU {[}1{]}  & Alibaba Cloud CDN                    & Computerline Group {[}757{]}                     \\
46 & HU              & KE {[}-1{]} & Apple Inc.                           & Eastlink (Delta) {[}1097{]}                      \\
47 & LT              & LT {[}0{]}  & CacheFly                             & Hivane {[}247{]}                                 \\
48 & LV              & LV {[}0{]}  & HUAWEI CLOUD                         & TIC AS49666 {[}1180{]}                           \\
49 & TR              & TR {[}0{]}  & Automattic                           & StarNet Moldova {[}961{]}                        \\
50 & EE & EE {[}0{]} & NetIX Communications Ltd.                          & DMC TECNOLOGIA E INFORMATICA {[}3717{]}                                    
\end{tabular}
\end{table}

==> tables/netcut_nodes_top30_tab.tex <==
%%avec betweenness
% \resizebox{0.99\textwidth}{!}{%
%     \begin{tabular}{@{}llll@{}}
%     \toprule
%       & Degree                    & Fitness                                   & Betweenness                         \\ \midrule
%     1  & Hurricane Electric        & Hurricane Electric {[}0{]}                & Hurricane Electric {[}0{]}          \\
%     2  & Cloudflare                & Packet Clearing House {[}1{]}             & Packet Clearing House {[}1{]}       \\
%     3  & Packet Clearing House     & Packet Clearing House AS42 {[}1{]}        & Cloudflare {[}-1{]}                 \\
%     4 &
%       Packet Clearing House AS42 &
%       Cloudflare {[}-2{]} &
%       Packet Clearing House AS42 {[}0{]} \\
%     5  & Google LLC                & Akamai Technologies {[}2{]}               & Google LLC {[}0{]}                  \\
%     6  & Microsoft                 & Google LLC {[}-1{]}                       & Akamai Technologies {[}1{]}         \\
%     7  & Akamai Technologies       & Microsoft {[}-1{]}                        & Facebook Inc {[}1{]}                \\
%     8  & Facebook Inc              & Facebook Inc {[}0{]}                      & Microsoft {[}-2{]}                  \\
%     9  & Amazon.com                & Amazon.com {[}0{]}                        & Amazon.com {[}0{]}                  \\
%     10 &
%       Netflix &
%       VeriSign Global Registry Services {[}5{]} &
%       EdgeCast Networks (VDMS) {[}2{]} \\
%     11 &
%       Yahoo! &
%       EdgeCast Networks (VDMS) {[}1{]} &
%       Netflix {[}-1{]} \\
%     12 &
%       EdgeCast Networks (VDMS) &
%       Netflix {[}-2{]} &
%       Limelight Networks Global {[}1{]} \\
%     13 & Limelight Networks Global & Limelight Networks Global {[}0{]}         & Yahoo! {[}-2{]}                     \\
%     14 & Fastly, Inc.              & Fastly, Inc. {[}0{]}                      & Fastly, Inc. {[}0{]}                \\
%     15 &
%       VeriSign Global Registry Services &
%       Yahoo! {[}-4{]} &
%       VeriSign Global Registry Services {[}0{]} \\
%     16 & G-Core Labs               & \textbf{Netnod} {[}11{]}                           & i3D.net {[}3{]}                     \\
%     17 & Apple Inc.                & Equinix Internet Exchange - MLPE {[}25{]} & \textbf{Netnod} {[}10{]}                     \\
%     18 & Riot Games                & i3D.net {[}1{]}                           & Apple Inc. {[}-1{]}                 \\
%     19 & i3D.net                   & \textbf{RIPE NCC K-Root Operations} {[}30{]}       & G-Core Labs {[}-3{]}                \\
%     20 & Blizzard Entertainment    & Salesforce.com {[}14{]}                   & Riot Games {[}-2{]}                 \\
%     21 & Subspace                  & Netskope {[}2{]}                          & Subspace {[}0{]}                    \\
%     22 & SG.GS                     & Subspace {[}-1{]}                         & Blizzard Entertainment {[}-2{]}     \\
%     23 & Netskope                  & \textbf{DNS-OARC-112} {[}29{]}                     & SG.GS {[}-1{]}                      \\
%     24 & Imperva                   & Riot Games {[}-6{]}                       & Netskope {[}-1{]}                   \\
%     25 & Twitch                    & Apple Inc. {[}-8{]}                       & Imperva {[}-1{]}                    \\
%     26 & Valve Corporation         & G-Core Labs {[}-10{]}                     & \textbf{RIPE NCC K-Root Operations} {[}23{]} \\
%     27 & Netnod                    & Twitch {[}-2{]}                           & Twitch {[}-2{]}                     \\
%     28 & Swisscom                  & Imperva {[}-4{]}                          & Quantil Networks {[}9{]}            \\
%     29 &
%       SoftLayer Technologies, Inc. &
%       Quantil Networks {[}8{]} &
%       StackPath (Highwinds) {[}1{]} \\
%     30 & StackPath (Highwinds)     & Blizzard Entertainment {[}-10{]}          & Swisscom {[}-2{]}                   \\ \bottomrule
%     \end{tabular}}
% \resizebox{0.99\textwidth}{!}{%
    \begin{tabular}{@{}llll@{}}
    \toprule
       & Degree                    & Fitness                                                       \\ \midrule
    1  & Hurricane Electric        & Hurricane Electric {[}0{]}                     \\
    2  & Cloudflare                & Packet Clearing House {[}1{]}                \\
    3  & Packet Clearing House     & Packet Clearing House AS42 {[}1{]}            \\
    4 &
      Packet Clearing House AS42 &
      Cloudflare {[}-2{]} \\
    5  & Google LLC                & Akamai Technologies {[}2{]}               \\
    6  & Microsoft                 & Google LLC {[}-1{]}                       \\
    7  & Akamai Technologies       & Microsoft {[}-1{]}                        \\
    8  & Facebook Inc              & Facebook Inc {[}0{]}                      \\
    9  & Amazon.com                & Amazon.com {[}0{]}                        \\
    10 &
      Netflix &
      VeriSign Global Registry Services {[}5{]}  \\
    11 &
      Yahoo! &
      EdgeCast Networks (VDMS) {[}1{]} \\
    12 &
      EdgeCast Networks (VDMS) &
      Netflix {[}-2{]}  \\
    13 & Limelight Networks Global & Limelight Networks Global {[}0{]}                              \\
    14 & Fastly, Inc.              & Fastly, Inc. {[}0{]}                                      \\
    15 &
      VeriSign Global Registry Services &
      Yahoo! {[}-4{]}  \\
    16 & G-Core Labs               & \textbf{Netnod} {[}11{]}                                 \\
    17 & Apple Inc.                & Equinix Internet Exchange - MLPE {[}25{]}                  \\
    18 & Riot Games                & i3D.net {[}1{]}                                      \\
    19 & i3D.net                   & \textbf{RIPE NCC K-Root Operations} {[}30{]}         \\
    20 & Blizzard Entertainment    & Salesforce.com {[}14{]}                             \\
    21 & Subspace                  & Netskope {[}2{]}                                  \\
    22 & SG.GS                     & Subspace {[}-1{]}                            \\
    23 & Netskope                  & \textbf{DNS-OARC-112} {[}29{]}                       \\
    24 & Imperva                   & Riot Games {[}-6{]}                          \\
    25 & Twitch                    & Apple Inc. {[}-8{]}                          \\
    26 & Valve Corporation         & G-Core Labs {[}-10{]}                     \\
    27 & Netnod                    & Twitch {[}-2{]}                            \\
    28 & Swisscom                  & Imperva {[}-4{]}                           \\
    29 &
      SoftLayer Technologies, Inc. &
      Quantil Networks {[}8{]}  \\
    30 & StackPath (Highwinds)     & Blizzard Entertainment {[}-10{]}        \\ \bottomrule
    \end{tabular}%}
